Markov Chain-based Optimization Time Analysis of Bivalent Ant Colony Optimization for Sorting and LeadingOnes

So far, only few bounds on the runtime behavior of Ant Colony Optimization (ACO) have been reported. To alleviate this situation, we investigate the ACO variant we call Bivalent ACO (BACO) that uses exactly two pheromone values. We provide and successfully apply a new Markov chain-based approach to calculate the expected optimization time, i. e., the expected number of iterations until the algorithm terminates. This approach allows to derive exact formulae for the expected optimization time for the problems Sorting and LeadingOnes. It turns out that the ratio of the two pheromone values significantly governs the runtime behavior of BACO. To the best of our knowledge, for the first time, we can present tight bounds for Sorting ($\Theta(n^3)$) with a specifically chosen objective function and prove the missing lower bound $\Omega(n^2)$ for LeadingOnes which, thus, is tightly bounded by $\Theta(n^2)$. We show that despite we have a drastically simplified ant algorithm with respect to the influence of the pheromones on the solving process, known bounds on the expected optimization time for the problems OneMax ($O(n\log n)$) and LeadingOnes ($O(n^2)$) can be re-produced as a by-product of our approach. Experiments validate our theoretical findings.

==> sections/runtime_analysis/onemax.tex <==
\subsection{OneMax}
In this section, the expected optimization time of \baco applied to the pseudo-boolean benchmark function \onemax is investigated.
\onemax maps a bit string of length $n$ to its number of ones:
$$\onemax(x)=\sum_{i=1}^{n} x_i$$

Typically the following construction graph $G$ is used for such pseudo-boolean objective functions (\cite{GUTJAHR20082711}, \cite{DOERR20111629}).
The starting node is connected to two nodes which denote the first bit of $x$ to be $0$ or $1$ respectively.
These two nodes are connected to a merge-node.
From here the same structure repeats for the second bit of $x$ etc.
This way an ant walking through $G$ builds up a path that is identified with a bit string.

Let the Markov states be the numbers from $0$ through $n$ which are identified with the \onemax function value of the current best solution.
Once state $n$ is reached the solution has been found and the algorithm terminates.
If the current state is $i\ne n$ then the probability to improve to state $i+1$ within one iteration is bounded from below as follows:
\begin{align}
	\Pr[i\rightarrow i+1]
	\ge(n-i)\cdot t\cdot\left(\frac{1}{1+t}\right)^n\label{eq:onemax_improve_by_one}
\end{align}
State $i+1$ can be reached as follows.
If the current state is $i$ then there are $n-i$ bits that are set to $0$.
Thus there are $n-i$ positions where the ant can deviate from the current best path and thereby flip a bit from $0$ to $1$.
The probability to deviate at exactly one of these positions multiplied by the total number of possible flips from $0$ to $1$ yields the lower bound~\eqref{eq:onemax_improve_by_one}.
Consequently the expected number of iterations until the state is improved from $i$ to $i+1$ is bound from above by the inverse of~\eqref{eq:onemax_improve_by_one}.
Thus summing up the expected number of iterations until the next state is reached for each Markov state (except $n$) yields an upper bound on the expected optimization time.
This allows to bound $T(n,t)$ as follows.
\begin{theorem}
	\label{thm:T_onemax_upper_bound}
	Let $t>0$ be the pheromone ratio.
	Then the expected optimization time of \baco for \onemax is upper bounded as follows:
	$$T(n,t)\le\frac{1}{t}\cdot(1+t)^n\cdot(1+\ln n)$$
	For the pheromone ratio $t=\frac{1}{n}$ this implies $T(n,t)\in\mathcal{O}(n\cdot\log n)$.
	\begin{proof}
		Assume the worst initial Markov state $0$ since this results in a larger expected number of iterations compared to the actual expected optimization time.
		Then restrict state changes to at most $1$ per iteration to further overestimate the expected number of iterations.
		This yields the following upper bound:
		\begin{align*}
			T(n,t)
			&\le\sum_{i=0}^{n-1} \Pr[i\rightarrow i+1]^{-1}
			\overset{\eqref{eq:onemax_improve_by_one}}{\le}
				\sum_{i=0}^{n-1}
				\left(\frac{1}{n-i}\cdot\frac{1}{t}\cdot(1+t)^n\right)\\
			&=
				\frac{1}{t}\cdot(1+t)^n
				\cdot\sum_{i=1}^{n} \frac{1}{i}
			\le
				\frac{1}{t}\cdot(1+t)^n
				\cdot(1+\ln n)
		\end{align*}
		The pheromone ratio $t=\frac{1}{n}$ yields the following:
		\begin{align*}
			T(n,t)
			&\le
				n\cdot\left(1+\frac{1}{n}\right)^n\cdot(1+\ln n)
			\le
				n\cdot e\cdot(1+\ln n)
			\in
				\mathcal{O}(n\cdot\log n)
		\end{align*}
	\end{proof}
\end{theorem}

